Search for Spatial Extension in High-Latitude Sources Detected by the Fermi Large Area Telescope

We present a search for spatial extension in high-latitude ($|b|>5^\circ$) sources in recent Fermi point source catalogs. The result is the Fermi High-Latitude Extended Sources Catalog, which provides source extensions (or upper limits thereof) and likelihood profiles for a suite of tested source morphologies. We find 24 extended sources, 19 of which were not previously characterized as extended. These include sources that are potentially associated with supernova remnants and star forming regions. We also found extended $\gamma$-ray emission in the vicinity of the Cen A radio lobes and - at GeV energies for the first time - spatially coincident with the radio emission of the SNR CTA 1, as well as from the Crab Nebula. We also searched for halos around active galactic nuclei, which are predicted from electromagnetic cascades that are induced by the $e^+e^-$ pairs that are deflected in intergalactic magnetic fields. These are produced when $\gamma$-rays interact with background radiation fields. We do not find evidence for extension in individual sources or in stacked source samples. This enables us to place limits on the flux of the extended source components, which are then used to constrain the intergalactic magnetic field a coherence length $\lambda \gtrsim 10\,$kpc, even when conservative assumptions on the source duty cycle are made. This improves previous limits by several orders of magnitude.

==> source_associations.tex <==
\section{Source Associations}

Here are some of the brief findings from Mattia and me : 

Source 1\newline
15	    306.07	SNR G295.5+09.7          	SNR	12 09 40.0 -52 25 00  \newline  	
Associated in SNR cat. \textbf{cite} \newline  	

Source 2: \newline
6 	    463.87	2MASX J00033726+6919064  	Galaxy  	00 03 37.261 +69 19 06.45 \newline  	

Source 3: \newline
221 	    376.58	HH 673B                         HH (8 - HerbigÐHaro (HH) objects) 	16 26 51.8 -24 38 37 \newline
Notes: $\sim$160 pc away \newline  	

Source 4: Near LMC\newline
PSR J0456-69. This one of LMC pulsars. \newline
162	    290.04	MQS J045529.15-691952.0       			AGN		04 55 29.150 -69 19 52.00  \newline
532	    569.15	ATPMN J045559.1-693329 (radio catalog)	AGN		04 55 59.100 -69 33 29.10  \newline
764	    692.41	NGC 1756                      			GlC (globular cluster)	 04 54 49.130 -69 14 10.20 \newline
Notes: 162 redshift = 0.413 \newline  	

Source 5: \newline
X-ray catalog \newline
22	    567.09	LkHa101CXO J043039.83+352146.1		G  	04 30 39.83 +35 21 46.1 \newline
27	    602.75	LkHa101CXO J043032.27+352218.5		G  	04 30 32.27 +35 22 18.5    	\newline
37	    662.91	LkHa101CXO J043025.19+352224.7		G  	04 30 25.19 +35 22 24.7    	\newline

Source 7: \newline
Nothing in the area from SIMBAD \newline
NVSS ... see table \newline  	

Source 8: \newline
1   	     15.48	[RHK2014] n1316 gc02965      	GlC	03 22 03.39 -37 14 34.0    	\newline
10  	     49.23	[RBD2012] 1061               	GlC	03 22 01.52 -37 15 12.1    	\newline
16  	     63.16	[RBD2012] 1075               	GlC	03 22 02.63 -37 13 20.9 \newline
20  	     77.71	[RHK2014] n1316 gc00662      	GlC	03 22 08.47 -37 13 56.0 \newline
29  	     98.28	[RBD2012] 2665               	GlC	03 22 01.24 -37 16 01.3    	\newline
É 177 globular clusters in ROI \newline

Source 9: \newline
Nothing in the area from SIMBAD \newline
NVSS ... see table \newline 	

Source 10: \newline
Nothing in the area from SIMBAD \newline
PMN ... see table (radio source) \newline  	

Source 11: \newline
6 	    412.08	[BDB2003] G117.56+06.15  	OpC (open galaxy cluster)	23 52 50.0 +68 24 30  \newline
NVSS ... see table \newline 	

Source 12: \newline
Nothing in the area from SIMBAD \newline
NVSS ... see table \newline   

Source 13: \newline
2 	    178.26	2MASX J07365880-3231053  	G  	07 36 58.810 -32 31 05.30 \newline  
6 	    368.96	GRB 941126B              	gB 	07 36 42.0 -32 35 00       \newline  
10	    439.37	2MASX J07364988-3226582  	G  	07 36 49.887 -32 26 58.26  	\newline  

Source 14: \newline
10 	    128.94	[CGC2008] J053526.84-660515.4 	G  	05 35 26.84 -66 05 15.4    	\newline
35 	    185.12	6dFGS gJ053601.0-660237       	G  	05 36 00.99 -66 02 36.6    	\newline
37 	    188.27	WHHW 0535.8-6604              	G  	05 35 44.6 -66 02 17       	\newline
46 	    198.40	NGC 2030                      	HII	05 35 33.6 -66 02 26       	\newline
50 	    203.15	2MASX J05354060-6602059       	G  	05 35 40.60 -66 02 05.9    	\newline
53 	    207.00	SNR B0535-66.0                	SNR	05 35 43.1 -66 01 59       	\newline
117	    310.04	DEM L 247                     	HII	05 36 28.0 -66 02 12       	\newline
125	    350.48	[CGC2008] J053519.13-660020.8 	G  	05 35 19.13 -66 00 20.8    	\newline
196	    614.25	2MASS J05371207-6559448       	G  	05 37 12.080 -65 59 44.81  	\newline

Source 15: \newline
Nothing in the area from SIMBAD \newline
NVSS ... see table \newline  

Source 16: Associated in 3FGL \newline

Source 17: Associated in 3FGL \newline 

Source 18: \newline
17	    638.15	GRB 060116               	gB 	05 38 46.170 -05 26 15.08 \newline
7 	    405.18	[OS98] 45                	Cld	05 39 42.0 -05 21 06\newline
5BZQ J0541-0541 \newline

Source 20: \newline
13	    697.50	UCAC4 631-018323             	Ro* (rotationally variable star??)	04 30 18.217 +36 01 34.18  	\newline

Source 21: \newline
101	    232.00	OGLE LMC178.5 10130           	AGN	05 38 07.900 -70 48 47.80  	\newline 
488	    533.35	MQS J053722.63-703719.3       	AGN	05 37 22.630 -70 37 19.30  	\newline
875	    707.73	2XMM J053600.4-704127         	Sy1	05 36 00.480 -70 41 27.70  	\newline


Source 22:  Associated in 3FGL \newline

Source 23: \newline
11	    325.52	SNR G332.5-05.6          	SNR	16 43 18.0 -54 30 00 \newline

Source 24: Associated in 3FGL \newline

Source 25: \newline
66 	    147.58	SNR J052559-660453            	SNR	05 26 00.4 -66 05 02       	\newline  
97 	    171.36	PSR B0525-66                  	Psr	05 26 00.7 -66 04 35       	\newline
453	    553.16	SNR B0525-66.0                	SNR	05 25 27.1 -65 59 11       	\newline  

Source 26: \newline
1 	     43.08	LEDA 2797400             	G  	02 37 56.3 +52 38 17       	\newline  
5 	    198.11	LEDA 2797398             	G  	02 37 55.1 +52 41 05    \newline  

Source 27: \newline
2 	    242.15	ESO 324-16               	G  	13 24 10.228 -39 15 46.99  	\newline   
5 	    475.30	6dFGS gJ132421.3-392343  	G  	13 24 21.258 -39 23 41.97  	\newline    
15	    692.84	[LH2011] 2117            	GrG	13 22 54.0 -39 20 00 \newline  
2MASSX see table \newline

Source 28: Associated in 3FGL \newline

Source 29: Associated in 3FGL\newline


==> theory.tex <==
\section{SOME BACKGROUND ON EXTENSIONS}\label{sec:theory}

\begin{figure}[ht]
\includegraphics[width=0.6\columnwidth]{./figures/PairHalos.png}
\caption{This is a figure. \label{fig:pair_halos}
\FIXME{MM: Do we really need this figure? We could simply reference to a review 
or one of the many papers where the underlying physics is discussed in greater detail.}
}
\end{figure}

\begin{table}[ht]
\begin{tabular}{c|c}
\hline \hline
Parameter & Result  \\ \hline

\end{tabular}
\caption{The world's greatest table
\label{tab:table}}
\end{table}


The library of templates will be developed using two independent, detailed simulation codes. 
The codes account for cosmological expansion, the EBL and CMB radiation fields, and all relevant QED cross section effects, in addition to performing the propagation of photons from any generic source spectrum through the universe to an observer~\cite{2014ApJ...796...18A}.
They contain accurate models of space as well as its relevant contents, and they propagate photons from a theoretically-motivated AGN ``source'' through the universe to an observer. Here are the details for two simulations. 

\subsection{ELMAG Simulations}\label{sec:simulations1}

The open-source ELMAG Monte Carlo code computes the 
observed photon flux (primary and cascade photons) 
using weighted sampling procedure 
(see Ref.~\cite{2012CoPhC.183.1036K} for details). 
Initial gamma rays are sampled
from an input spectrum, which we set 
to be a power law with index $\Gamma = 2$. 
Interactions with the CMB and EBL are taken into account, 
and all secondary particles with an 
energy $\epsilon \geq \epsilon_\mathrm{thr}$ 
are traced, i.e. we set the sampling factor $\alpha_\mathrm{sample} = 0$.
Energy losses due to inverse-Compton scattering and synchrotron radiation
are integrated out for $\epsilon < \epsilon_\mathrm{thr}$ 
and we set $\epsilon_\mathrm{thr} = 100\,$MeV. 
ELMAG adopts a simplified description of the IGMF,
namely that its field strength is constant 
and its orientation changes randomly in cells whose 
length is equal to the coherence length. 
In each coherence-length patch, the $B$ field is assumed to be perpendicular 
to the particle trajectory. 
Within ELMAG, the small-angle approximation is adopted
and the observation angle of the cascade photons is randomized once 
the total squared deflection angle exceeds $\pi^2 / 4$.
As a result, ELMAG results for large magnetic fields and / or 
large deflections have to be treated with care.
We use the EBL model of Ref. \cite{Dominguez:2010bv} 
and test different jet opening angles,
$\theta_\mathrm{jet} = 1^\circ, 3^\circ, 6^\circ, 10^\circ$, 
where it is assumed that the bulk Lorentz factor 
of the emitting plasma is given by $\Gamma_\mathrm{L} = \theta_\mathrm{jet}^{-1}$. 
We simulate the full cascade spectrum over a grid of 
redshifts in bins of injected gamma-ray energy $\Delta E_i$ between 100\,MeV and 32\,TeV (using again 8 bins per decade). 
This enables us to model any injected gamma-ray spectrum $\phi(E)$
by reweighting the cascade spectrum caused by injected gamma-rays whose 
energy $E \in \Delta E_i$ with a weight $w_i$:
\begin{equation}
w_i = \frac{\int\limits_{\Delta E_i} dE\, \phi(E) }{\int\limits_{\Delta E_i} dE\, E^{-2}}.
\end{equation}


\subsection{Brendan's Simulations}\label{sec:simulations2}

Details and contrasts of Brendan's Simulations. Include a figure. 

